LogShrink: Effective Log Compression by Leveraging Commonality and Variability of Log Data

Log data is a crucial resource for recording system events and states during system execution. However, as systems grow in scale, log data generation has become increasingly explosive, leading to an expensive overhead on log storage, such as several petabytes per day in production. To address this issue, log compression has become a crucial task in reducing disk storage while allowing for further log analysis. Unfortunately, existing general-purpose and log-specific compression methods have been limited in their ability to utilize log data characteristics. To overcome these limitations, we conduct an empirical study and obtain three major observations on the characteristics of log data that can facilitate the log compression task. Based on these observations, we propose LogShrink, a novel and effective log compression method by leveraging commonality and variability of log data. An analyzer based on longest common subsequence and entropy techniques is proposed to identify the latent commonality and variability in log messages. The key idea behind this is that the commonality and variability can be exploited to shrink log data with a shorter representation. Besides, a clustering-based sequence sampler is introduced to accelerate the commonality and variability analyzer. The extensive experimental results demonstrate that LogShrink can exceed baselines in compression ratio by 16% to 356% on average while preserving a reasonable compression speed.

==> sections/backup.tex <==

\subsection{Motivation}
A statistics result of relation E-H, E-E and V-V is shown in Table.~\ref{tab:relation_stat}. For E-H, we define a relation between event and header is that whether a header value changes in one log event. The first row in table presents the average count of header field that have a relation with log event. The second row in table presents the percentage of these headers fields.  We can observe that %there are
23\%$\sim$43\% of headers have relations with log event. The most case is Android, which takes 43\% of all header fields\hy{how to see it from Table 1?}. The results show that relations exist between log events and headers. 



\subsection{Relation Miner}

% the motivation to use markov chain and state machine

% introduce markov chain first
we first give introduction of Markov chain and state transition matrix.
Markov chain is widely used in temporal series analysis.
A markov chain is a stochastic model describing a sequence of possible events in which the probability of each events depends only on the state attained in the previous event.
% introduce state transmition matrix
Given finite possible event set, we define each possible event as a state. The transition matrix of the Markov chain is $P=(p_{ij})$. $p_{ij}$ is the transition probability of state $i$ to state $j$, where state $i$ belongs to the state set $S_1$ and state $j$ belongs to the state set $S_2$. Note that $p_{ij} \leq 0$ for all $i$, and satisfy the condition in Equation.~\ref{eq:transition_matrix_cond}.
\begin{equation}
\label{eq:transition_matrix_cond}
    \sum_{k=1}^r p_{i k}=\sum_{k=1}^r P\left(X_{m+1}=k \mid X_m=i\right)=1
\end{equation}
% Should we give a definition of relation here?

% how to calculate state transmition matrix
We aggregate all the possible transition in a series and then calculate the transition matrix.
% how to define there exists a relation
Based on the transition matrix, we define a relation exists between state $i$ and state $j$ if $p_{ij} > \sigma$. The $\sigma$ is a pre-defined threshold. Then we calculate a relation set following the Equation.~\ref{eq:relation_set}.

% TODO: check the correctness of this equation
\begin{equation}
\label{eq:relation_set}
R = \{(i, j) | p_{ij} > \sigma, i \in S_1, j \in S_2\}
\end{equation}

The above basic relation miner is applied in pairs of log components to mine relations. But we need to define the states carefully in each application as we discuss in the following.

\begin{itemize}
    \item E-H. We define the set of log event as state set $S_1$ and the set of each log headers as state set $S_2$. 
    \item E-E. Considering a series of log events $E = \{e_1, e_2, ..., e_l\}$. N-gram refers to a contiguous subsequence of n items from a sequence. We define the set of n-gram log event (e.g., $(e_1, ..., e_n)$ as state set $S_1$ and the set of next item as state set $S_2$.
    \item V-V. Given a variable set $V=\{v_{{e_1}1}, v_{{e_1}2}, ..., v_{{e_n}m}\}$, where $v_{{e_n}m}$ refers to the $m_{th}$ variable in log event $e_n$. To mine relations between variables, the state set $S_1$ and $S_2$ are referred to the variable set $V$.
    \item E-V. We define the set of log event as state set $S_1$ and the variable set $V$ as state set $S_2$. % E-V is a different type
\end{itemize}



==> sections/related_work.tex <==
\section{Related work}
Data compression generally includes lossless compression and lossy compression. We focus on lossless compression in this paper. 


\textbf{General-purpose data compression methods.} These algorithms usually exploit statistical redundancy to eliminate redundancy literally, which can be categorized as three types: entropy-based, dictionary-based, and predict-based. Entropy-based methods (e.g., Huffman encoding~\cite{huffman1952method}, Arithmetic encoding~\cite{witten1987arithmetic}) build a probability model and find the optimal minimize coding for data. Dictionary-based methods (e.g., gzip, lzma) search the repeated tokens and replace them with dictionary references when processing the input stream. Predict-based methods (e.g., PPMd~\cite{cleary1984data}, DeepZip~\cite{goyal2018deepzip}) use a set of previous tokens to predict the next token, and encode the prediction results adaptively.

\textbf{Log-specific data compression methods.} Considering log data as semi-structured data, it is highly redundant by nature. These methods are categorized as two types: non-parser based and parser based. Non-parser based log compression methods (e.g., CLC, LogArchive~\cite{christensen2013adaptive}, Cowic~\cite{lin2015cowic} and MLC~\cite{feng2016mlc}) process log data without pattern extraction.
Parser-based log compression methods~\cite{liu2019logzip,ding2021elise,yao2021improving,wei2021feasibility} use a log parser to extract templates and process headers, templates, and variables separately. According to the data type, they apply different encoding methods like delta encoding, common sub-pattern extraction, dictionary encoding to shrink log data in column manner. In terms of relation utilization, parser-based log compression methods mines relation between log lines. LogReducer~\cite{wei2021feasibility} further compresses numerical variables by mining numerical relation inline and an elastic encoder. But it cannot mine relations across lines.
CLP~\cite{rodrigues2021clp} and LogGrep~\cite{wei2023loggrep} deliver efficient query tools on compressed data. CLP parses log lines into schema and store the variables as dictionary variables and non-dictionary variables. LogGrep further extracts static patterns and runtime patterns of dictionary variables and packs them into a set of capsules in fine-grained. But they could not achieve a high compression ratio while preserving searchable features.  


% preprocessing: delta encoding on timestamp, dictionary encoding on string values, extracting common prefix
% 

\textbf{Relation analyzing in log data. } Relation analyzing in log data is widely used in other log analysis task like anomaly detection. The key of anomaly detection task is to find the outlier of all data, so they~\cite{lou2010mining, zhang2020anomaly} generally mine workflows on log events instead of mining relations in log headers and log variables. Lou et al.~\cite{lou2010mining} mine constant liner relationships in log event occurrence to identify invariants and then detect anomalies when the incoming log deviates from existing invariants. 

\hy{the paper writing (including English usage) should be significantly improved.}
